Attending Form and Context to Generate Specialized Out-of-VocabularyWords Representations

We propose a new contextual-compositional neural network layer that handles out-of-vocabulary (OOV) words in natural language processing (NLP) tagging tasks. This layer consists of a model that attends to both the character sequence and the context in which the OOV words appear. We show that our model learns to generate task-specific \textit{and} sentence-dependent OOV word representations without the need for pre-training on an embedding table, unlike previous attempts. We insert our layer in the state-of-the-art tagging model of \citet{plank2016multilingual} and thoroughly evaluate its contribution on 23 different languages on the task of jointly tagging part-of-speech and morphosyntactic attributes. Our OOV handling method successfully improves performances of this model on every language but one to achieve a new state-of-the-art on the Universal Dependencies Dataset 1.4.

==> acknowledgements.tex <==
\section*{Acknowledgments}

==> qualitative_comparison_it.tex <==
\begin{table*}[h!]
\small
\centering
\begin{tabular}{p{15cm}}
\toprule
\textbf{POS}: {\transparent{0.1505}\colorbox{red}{\transparent{1.0}{{\strut lo}}}} {\transparent{0.1527}\colorbox{red}{\transparent{1.0}{{\strut storico}}}} {\transparent{0.1537}\colorbox{red}{\transparent{1.0}{{\strut ,}}}}
\textbf{[{\transparent{0.1431}\colorbox{red}{\transparent{1.0}{{\strut p}}}}{\transparent{0.0099}\colorbox{red}{\transparent{1.0}{{\strut a}}}}{\transparent{0.2444}\colorbox{red}{\transparent{1.0}{{\strut t}}}}{\transparent{0.1714}\colorbox{red}{\transparent{1.0}{{\strut e}}}}{\transparent{0.2009}\colorbox{red}{\transparent{1.0}{{\strut r}}}}{\transparent{0.1883}\colorbox{red}{\transparent{1.0}{{\strut n}}}}{\transparent{0.118}\colorbox{red}{\transparent{1.0}{{\strut a}}}}{\transparent{0.2257}\colorbox{red}{\transparent{1.0}{{\strut l}}}}{\transparent{0.14}\colorbox{red}{\transparent{1.0}{{\strut i}}}}{\transparent{0.2156}\colorbox{red}{\transparent{1.0}{{\strut s}}}}{\transparent{0.2297}\colorbox{red}{\transparent{1.0}{{\strut t}}}}{\transparent{0.1364}\colorbox{red}{\transparent{1.0}{{\strut i}}}}{\transparent{0.1458}\colorbox{red}{\transparent{1.0}{{\strut c}}}}{\transparent{0.1309}\colorbox{red}{\transparent{1.0}{{\strut o}}}}]}
{\transparent{0.1535}\colorbox{red}{\transparent{1.0}{{\strut disinteresse}}}} {\transparent{0.154}\colorbox{red}{\transparent{1.0}{{\strut di}}}} {\transparent{0.1537}\colorbox{red}{\transparent{1.0}{{\strut la}}}} {\transparent{0.1526}\colorbox{red}{\transparent{1.0}{{\strut chiesa}}}} {\transparent{0.1494}\colorbox{red}{\transparent{1.0}{{\strut cattolica}}}} {\transparent{0.1535}\colorbox{red}{\transparent{1.0}{{\strut verso}}}} {\transparent{0.1535}\colorbox{red}{\transparent{1.0}{{\strut il}}}} {\transparent{0.1533}\colorbox{red}{\transparent{1.0}{{\strut loro}}}} {\transparent{0.1535}\colorbox{red}{\transparent{1.0}{{\strut "}}}} {\transparent{0.1466}\colorbox{red}{\transparent{1.0}{{\strut genio}}}} {\transparent{0.1537}\colorbox{red}{\transparent{1.0}{{\strut "}}}} {\transparent{0.1516}\colorbox{red}{\transparent{1.0}{{\strut è}}}} {\transparent{0.1537}\colorbox{red}{\transparent{1.0}{{\strut a}}}} {\transparent{0.1535}\colorbox{red}{\transparent{1.0}{{\strut la}}}} {\transparent{0.1536}\colorbox{red}{\transparent{1.0}{{\strut fine}}}} {\transparent{0.1534}\colorbox{red}{\transparent{1.0}{{\strut .}}}}
\\
\textbf{MORPH}: {\transparent{0.2077}\colorbox{red}{\transparent{1.0}{{\strut lo}}}} {\transparent{0.1874}\colorbox{red}{\transparent{1.0}{{\strut storico}}}} {\transparent{0.1707}\colorbox{red}{\transparent{1.0}{{\strut ,}}}}
\textbf{[{\transparent{0.1839}\colorbox{red}{\transparent{1.0}{{\strut p}}}}{\transparent{0.3202}\colorbox{red}{\transparent{1.0}{{\strut a}}}}{\transparent{0.7832}\colorbox{red}{\transparent{1.0}{{\strut t}}}}{\transparent{0.008}\colorbox{red}{\transparent{1.0}{{\strut e}}}}{\transparent{0.0003}\colorbox{red}{\transparent{1.0}{{\strut r}}}}{\transparent{0.0028}\colorbox{red}{\transparent{1.0}{{\strut n}}}}{\transparent{0.0002}\colorbox{red}{\transparent{1.0}{{\strut a}}}}{\transparent{0.0005}\colorbox{red}{\transparent{1.0}{{\strut l}}}}{\transparent{0.0001}\colorbox{red}{\transparent{1.0}{{\strut i}}}}{\transparent{0.0002}\colorbox{red}{\transparent{1.0}{{\strut s}}}}{\transparent{0.0002}\colorbox{red}{\transparent{1.0}{{\strut t}}}}{\transparent{0.0}\colorbox{red}{\transparent{1.0}{{\strut i}}}}{\transparent{0.0002}\colorbox{red}{\transparent{1.0}{{\strut c}}}}{\transparent{0.0}\colorbox{red}{\transparent{1.0}{{\strut o}}}}]}
{\transparent{0.1622}\colorbox{red}{\transparent{1.0}{{\strut disinteresse}}}} {\transparent{0.1612}\colorbox{red}{\transparent{1.0}{{\strut di}}}} {\transparent{0.1551}\colorbox{red}{\transparent{1.0}{{\strut la}}}} {\transparent{0.1525}\colorbox{red}{\transparent{1.0}{{\strut chiesa}}}} {\transparent{0.152}\colorbox{red}{\transparent{1.0}{{\strut cattolica}}}} {\transparent{0.1509}\colorbox{red}{\transparent{1.0}{{\strut verso}}}} {\transparent{0.1502}\colorbox{red}{\transparent{1.0}{{\strut il}}}} {\transparent{0.1496}\colorbox{red}{\transparent{1.0}{{\strut loro}}}} {\transparent{0.1508}\colorbox{red}{\transparent{1.0}{{\strut "}}}} {\transparent{0.1498}\colorbox{red}{\transparent{1.0}{{\strut genio}}}} {\transparent{0.1505}\colorbox{red}{\transparent{1.0}{{\strut "}}}} {\transparent{0.1508}\colorbox{red}{\transparent{1.0}{{\strut è}}}} {\transparent{0.1492}\colorbox{red}{\transparent{1.0}{{\strut a}}}} {\transparent{0.1404}\colorbox{red}{\transparent{1.0}{{\strut la}}}} {\transparent{0.0085}\colorbox{red}{\transparent{1.0}{{\strut fine}}}} {\transparent{0.0005}\colorbox{red}{\transparent{1.0}{{\strut .}}}}
\\
\bottomrule
\end{tabular}
\caption{Attention results on both tasks for the same Italian sentence.}\label{tab:qualitative_comparison_it}
\end{table*}

==> qualitative_comparison_ru.tex <==
\begin{table*}[h!]
\small
\centering
\begin{tabular}{c}
% \begin{tabular}{p{7cm}}
\toprule
\textbf{POS}: \foreignlanguage{russian}{
{\transparent{0.2331}\colorbox{red}{\transparent{1.0}{{\strut Недалеко}}}} {\transparent{0.2365}\colorbox{red}{\transparent{1.0}{{\strut от}}}}
\textbf{[{\transparent{0.159}\colorbox{red}{\transparent{1.0}{{\strut д}}}}{\transparent{0.2702}\colorbox{red}{\transparent{1.0}{{\strut а}}}}{\transparent{0.321}\colorbox{red}{\transparent{1.0}{{\strut о}}}}{\transparent{0.162}\colorbox{red}{\transparent{1.0}{{\strut с}}}}{\transparent{0.1686}\colorbox{red}{\transparent{1.0}{{\strut к}}}}{\transparent{0.2881}\colorbox{red}{\transparent{1.0}{{\strut о}}}}{\transparent{0.2083}\colorbox{red}{\transparent{1.0}{{\strut г}}}}{\transparent{0.2228}\colorbox{red}{\transparent{1.0}{{\strut о}}}}]}
{\transparent{0.2198}\colorbox{red}{\transparent{1.0}{{\strut храма}}}} {\transparent{0.1542}\colorbox{red}{\transparent{1.0}{{\strut Чэнхуанмяо}}}} {\transparent{0.2353}\colorbox{red}{\transparent{1.0}{{\strut раньше}}}} {\transparent{0.2434}\colorbox{red}{\transparent{1.0}{{\strut находился}}}} {\transparent{0.2363}\colorbox{red}{\transparent{1.0}{{\strut рынок}}}} {\transparent{0.2415}\colorbox{red}{\transparent{1.0}{{\strut .}}}}
}\\
\textbf{MORPH}: \foreignlanguage{russian}{
{\transparent{0.2318}\colorbox{red}{\transparent{1.0}{{\strut Недалеко}}}} {\transparent{0.2183}\colorbox{red}{\transparent{1.0}{{\strut от}}}}
\textbf{[{\transparent{0.1695}\colorbox{red}{\transparent{1.0}{{\strut д}}}}{\transparent{0.1793}\colorbox{red}{\transparent{1.0}{{\strut а}}}}{\transparent{0.1928}\colorbox{red}{\transparent{1.0}{{\strut о}}}}{\transparent{0.1753}\colorbox{red}{\transparent{1.0}{{\strut с}}}}{\transparent{0.2686}\colorbox{red}{\transparent{1.0}{{\strut к}}}}{\transparent{0.2401}\colorbox{red}{\transparent{1.0}{{\strut о}}}}{\transparent{0.3366}\colorbox{red}{\transparent{1.0}{{\strut г}}}}{\transparent{0.2379}\colorbox{red}{\transparent{1.0}{{\strut о}}}}]}
{\transparent{0.2142}\colorbox{red}{\transparent{1.0}{{\strut храма}}}} {\transparent{0.2501}\colorbox{red}{\transparent{1.0}{{\strut Чэнхуанмяо}}}} {\transparent{0.2189}\colorbox{red}{\transparent{1.0}{{\strut раньше}}}} {\transparent{0.2141}\colorbox{red}{\transparent{1.0}{{\strut находился}}}} {\transparent{0.2272}\colorbox{red}{\transparent{1.0}{{\strut рынок}}}} {\transparent{0.2254}\colorbox{red}{\transparent{1.0}{{\strut .}}}}
}\\
\bottomrule
\end{tabular}
\caption{Attention results on both tasks for the same Russian sentence.}\label{tab:qualitative_comparison_ru}
\end{table*}
